Addressing Negative Transfer in Diffusion Models

Diffusion-based generative models have achieved remarkable success in various domains. It trains a shared model on denoising tasks that encompass different noise levels simultaneously, representing a form of multi-task learning (MTL). However, analyzing and improving diffusion models from an MTL perspective remains under-explored. In particular, MTL can sometimes lead to the well-known phenomenon of negative transfer, which results in the performance degradation of certain tasks due to conflicts between tasks. In this paper, we first aim to analyze diffusion training from an MTL standpoint, presenting two key observations: (O1) the task affinity between denoising tasks diminishes as the gap between noise levels widens, and (O2) negative transfer can arise even in diffusion training. Building upon these observations, we aim to enhance diffusion training by mitigating negative transfer. To achieve this, we propose leveraging existing MTL methods, but the presence of a huge number of denoising tasks makes this computationally expensive to calculate the necessary per-task loss or gradient. To address this challenge, we propose clustering the denoising tasks into small task clusters and applying MTL methods to them. Specifically, based on (O2), we employ interval clustering to enforce temporal proximity among denoising tasks within clusters. We show that interval clustering can be solved using dynamic programming, utilizing signal-to-noise ratio, timestep, and task affinity for clustering objectives. Through this, our approach addresses the issue of negative transfer in diffusion models by allowing for efficient computation of MTL methods. We validate the efficacy of proposed clustering and its integration with MTL methods through various experiments, demonstrating 1) improved generation quality and 2) faster training convergence of diffusion models.

==> contents/6_limitations.tex <==



==> contents/backup.tex <==
% Diffusion-based generative models~\cite{ho2020denoising, sohl2015deep, song2021scorebased} have accomplished remarkable success in various image generation settings, including unconditional~\cite{karras2022elucidating, nichol2021improved}, class-conditional~\cite{ho2022cascaded}, and text-conditional~\cite{balaji2022ediffi, nichol2022glide, ramesh2022hierarchical} generation.
% They can outperform the quality of GANs~\cite{goodfellow2020generative} in a specific condition and are rapidly applied to other domains including video generation~\cite{ho2022imagen, ho2022video}, natural language generation~\cite{li2022diffusion}, and 3D generation~\cite{poole2022dreamfusion, luo2021diffusion}.
% Consequently, improving the diffusion model has garnered significant interest.

% \shinhyeok{It trains a model on denoising tasks over various noise levels simultaneously, which can be interpreted as multi-task learning (MTL) if we assume that the denoising task about each noise level is a single task.}
% \shinhyeok{The model is trained concurrently on denoising tasks across multiple noise levels, which, under the assumption that each noise level represents a distinct task, can be construed as an instance of multi-task learning (MTL).}
% \shinhyeok{The technique involves training a model to perform denoising tasks across multiple levels of noise concurrently. This can be viewed as an instance of multi-task learning (MTL) under the assumption that each denoising task for a given noise level represents a distinct task.}

% Based on these observations, our second set of contributions aims to improve diffusion training by addressing negative transfer. However, adapting existing MTL methods for a large set of denoising tasks in diffusion training can be computationally expensive since per-task loss and gradient computations must be performed in each iteration. To overcome this issue, we propose to cluster denoising tasks and apply MTL methods to the clustered tasks. We use an interval clustering approach with constraints based on the adjacency of noise levels and timesteps, as observed in our second observation of the task affinity score. By clustering similar tasks, our proposed approach can reduce the computational burden and improve the overall performance of the diffusion model.



% In this work, we aim to analyze and improve diffusion training from MTL aspects.
% As our first contribution, we conduct an observational study to investigate the nature of diffusion training as a multi-task learning problem. 
% Through our analysis, we make two key observations.
% First, we observe that \textit{negative transfer} also exists in diffusion training, resulting in performance degradation due to its inherent multi-task learning scheme.
% Second, we analyze the relation between denoising tasks by using the task affinity score that is known as correlated with the performance of jointly trained model~\cite{azorin2023s, fifty2021efficiently}.
% The task affinity score decreases as the distance between noise level and timestep, indicating that the performance of the jointly learned model may be more degraded.









% \hist{written by ChatGPT}
% The Diffusion Model is a powerful machine learning approach used for tackling unbalanced tasks. Its total objective involves the weighted summation of loss at each diffusion time-step, and various strategies such as loss weighting and multi-expert approaches have been proposed to improve Diffusion training within this objective. These methods have proven effective in improving various metrics.

% In our paper, we aim to explore the effectiveness of Multi-task learning (MTL) methodology in Diffusion training. In MTL, tasks are balanced based on heuristics that consider the differences between them, such as loss scale or other factors. We demonstrate that these approaches can be used to perform P2 weight and MinSNR balancing in Diffusion. Furthermore, we investigate the use of the multi-expert approach in MTL, which is commonly used in Single Task Learning.

% However, we discovered that the Gradient Conflict problem, a common issue in MTL, persists in Diffusion. Gradient Conflict refers to the conflict between the gradients of different tasks during the optimization process, which can negatively impact performance. To address this issue, we aim to bring Gradient Conflict resolution methods into Diffusion training. The most challenging part of this is obtaining per-task gradients, which requires K-step forward and backward computations. To overcome this challenge, we propose clustering the continuous Diffusion task into K smaller tasks. This approach allows us to obtain per-task gradients and improve the performance of the Diffusion Model.

% In summary, our paper aims to demonstrate the effectiveness of MTL methodology in Diffusion training and address the Gradient Conflict problem. By proposing a novel approach to clustering the continuous Diffusion task into smaller tasks, we aim to obtain per-task gradients and improve the performance of the Diffusion Model.
 
% -----------


% - Diffusion Model은 센세이션입니다.
% - Unbalanced Task.
% - Diffusion model의 total objective는 각각의 diffusion time-step의 loss가 weighted summation되는 구조입니다.
    % 1. forward-time diffusion process
        
    %     $$
    %     x_{t+1}= \sqrt{1-\beta_t}x_t + \beta_t\epsilon_t
    %     $$
        
    % 2. 여기에서 continuous limit에서는 diffusion process는:
        
    %     $$
    %     dx_t = f(x_t, t)dt + g(t)dw_t
    %     $$
        
        % with $t$ being a continuum of the diffusion index in [0, T], 위에 f랑 g는 drift랑 volatility coefficient임.
        
    % 3. 이거 reverse diffusion process.
        
    %     $$
    %     dx_t=[f(x_t,t)-g^2(t)\log{p_r^t(x_t)}]d\overline{t} + g(t)d\overline{w_t}
    %     $$
        
    % 4. diffusion trains a score network $s_\theta$
    
    % $$
    % L=\frac{1}{2}\int_0^T{\xi(t)}\mathbb{E}[||s_\theta(x_t,t)-\nabla\log{p_r^t}(x_t)||_2^2] dt
    % $$
    
% - 이러한 Objective에서 Diffusion Training을 발전시키기 위해서 다음과 같은 전략들이 사용되어 왔습니다.
%     1. Loss weighting:  $\xi(t)$를 그들만의 heuristic으로 변경시키는 것들을 제안한 work. \hist{인용 없음}
%     2. Multi-expert: Diffusion index $t=[0,T]$ 를 몇등분 하여 specific 한 time step에 specialized된 모델을 사용하는 방법. \hist{인용 없음 (ediff-i 랑 ppap?)}
% - 이들 방법은 정말 효과적이었고, 여러 Metric을 올리는데 기여를 할 수 있었습니다.
% - 여기서, 우리는 이러한 방법들의 효과를 Multi-task learning 관점에서 이해할 수 있음을 보일것임.
%     - MTL에서의 Loss weighting: Loss의 Scale등이 다른 것들을 고려하여 heuristic 기반으로 Task를 밸런싱함. → 이거 기준으로 P2 weight, MinSNR balancing을 할 수 있음을 보임.
%     - Multi-expert: MTL에서 가장 많이 쓰이는 Single Task Learning을 의미함.
% - 이러한 Approach를 이해한뒤에 우리는 Diffusion에서도 MTL에서 큰 문제인 Conflict Gradient들이 남아있다는 것을 발견할거임. (있는지는 몰?루? 아마 있을것으로 생각함 지금 결과로는.)
%     - Ex) Loss weighting은 gradient의 conflict는 해결하지 못함.
%     - Ex) Multi-expert는 Parameter의 개수가 너무 늠.
% - 우리는 이것을 해결하기 위해 Gradient Conflict 해결방법을 가져오는 게 목표임.
%     - 여기서 가장 Challenge한 부분은 Per-task gradient를 구하는 것인데, 이는 K-step forward K-step backward가 필요함.
%     - Diffusion의 Continous한 Task를 작은 K개로 나누는 것으로 이를 해결함.
%         - clustering하나.
% - (Concurrent work으로 이를 multi-task learning으로 봐서 Pareto optimality를 위한 weight를 Optimize하는 방법이 나왔지만, 우리는 multi-task learning 방법론을 들고오는 것을 목표로 합니다.)


% \hist{related work 과 preliminary 를 구분해야합니다. 여기 적을 거라고 써놓은 내용들은 지금 보기엔 related work 보다는 preliminray 에 가까워 보입니다. related work 에서는 우리 연구와 "비교해야할만한" 연구 들에 대해서 소개하고, 그 연구들과의 차이점을 위주로 설명해야 합니다.}

% \hyojun{저는 둘다 포함하려고했어여, 우리 연구와 관련한 연구들을 설명하고, 이중에서 우리의 포지션과 차이점들을 설명하려고 했습니다!}

% In this section, we briefly review the related works and the relation between them and our works.

% The closest study to ours is MinSNR~\cite{hang2023efficient} since they and we have a common insight that diffusion training is multi-task learning.
% In contrast to this, we further investigate the multi-task learning nature in diffusion models by observing negative transfer and task affinity.
% Also, we enable to apply of well-established multi-task learning methods for diffusion models by clustering entire denoising tasks to small groups, which failed in MinSNR since instability and inefficiency. 


% Also, we will show that our methodology is readily applicable to these improved training objectives.
% \hyojun{이 문장에 대한 실험이 아직 안되어있어여.}

% \hyojun{이 부분 밑에 Gradient conflict, magnitude, imbalance이거 잘 적어줘야하는 것 같음여.}

% First, to deal with conflicting gradients between tasks, PC-grad~\cite{yu2020gradient} and Graddrop~\cite{chen2020just} mitigate this by projecting conflicting parts of gradients and dropping elements of gradients  based on the degree of conflict, respectively.

% Second, to address differences in gradient magnitudes, various optimization methods have been proposed to equalize them, such as MGDA-UB~\cite{sener2018multi}, IMTL-G~\cite{liu2021towards}, and NashMTL~\cite{navon2022multi}.

% Third, several methods have been proposed to balance task losses by using uncertainty~\cite{kendall2018multi}, task difficulty~\cite{guo2018dynamic}, and gradient norm~\cite{chen2018gradnorm} to mitigate the unbalanced scale between task losses.

% In this work, we observe negative transfer in diffusion training and argue addressing it as a direction to improve diffusion models.

% Our objective is to address these challenges and apply them to diffusion models.



% that diffusion training suffers from negative transfer and argue that mitigating it is the feasible direction to improve diffusion models.
% However, MTL methods mainly target scenarios with a small number of tasks and easily measurable individual task performance, which makes adapting negative transfer and applying MTL methods to diffusion models challenging.



% \textbf{Task Groupings}
% In the early attempt to identify the proper task grouping for better performance, an exhaustive cross-validation procedure that evaluates all task combinations is explored~\cite{standley2020tasks},
% However, this procedure requires huge computational cost, thus several works explore task affinity scores, such as gradient similarity and changes in task losses after the parameter update, to group tasks based on their correlation with the performance of the jointly learned model~\cite{fifty2021efficiently,azorin2023s}.
% In our work, we utilize a gradient direction-based task affinity score to analyze affinity between denoising tasks.


% In our work, we use gradient direction-based task affinity score to analyze the relationship between tasks, which has been shown to be effective in previous works~\cite{fifty2021efficiently, azorin2023s}.
% Also, 



% Unlike these tasks that generate a set of tasks, our method groups timesteps into a set of intervals, and we also perform clustering based on parameters present in the diffusion.
% 
% Other work~\cite{song2022efficient} aims to learn it by the meta-learning scheme.





% To identifying the proper task grouping for producing better results, the early attempts~\cite{standley2020tasks} run intensive cross-validation procedure for all task combinations.
% However, this procedure requires huge computational cost, thus works define task affinity scores to correlate the performance of jointly learned model and group tasks by using task affinity scores
% ~\cite{fifty2021efficiently,azorin2023s}.
% Furthermore, recent work~\cite{song2022efficient} apply meta-learning to learn task affinity for multi-task grouping.

% For $0\leq s \leq t \leq T$, let $\alpha_{t|s}=\alpha_t/\alpha_s$ and $\text{SNR}(t)$ decrease from $t=0$ to $t=T$ with $q(\mathbf{x}_T) \approx \mathcal{N(\textbf{0}, \textbf{I})}$.


% \doni{$\text{SNR}(t)$ decrease from $\text{SNR}(0)=1$ to $\text{SNR}(T)=0$ 은 어떤가요}
% \hyojun 좋은 의견인데, SNR이 Diffusion 모델마다 다릅니다!

% \hyojun{승현님: O1, O2 switching하자. O2 가 O1의 grouping동기를 내포하고 있는 것 같다.}
% \hyojun{
% 3.2에서 "우리가 3.1에서 theoretically MTL 임을 보였고, 이걸 empirically 확인해보기 위해서 research question 2개를 던져봤다. 
% 1) jointly 학습하는게 하나씩 따로 학습하는 것보다 성능이 떨어지는가? 
% 2) 1000개 태스크는 너무 많은데, 이걸 줄일 수는 없을까?" 같은 걸로 풀어나가는건 어떨까 하는 생각이
% }


% To investigate the multi-task learning nature in the diffusion models, we experimentally analyze them with two aspects: 
% 1) Task affinity: the relationship between denoising tasks.
% the similarity between gradient directions of denoising tasks across training iterations, which correlated to the performance of a jointly learned model on tasks,
% 2) Negative transfer: performance degradation caused by multi-task learning in diffusion models.
% We use a lightweight ADM~\cite{dhariwal2021diffusion} used in~\cite{choi2022perception} and LDM~\cite{rombach2022high} with FFHQ 256$\times$256 dataset~\cite{karras2019style} for analyze diffusion models trained on both pixel and latent space.
% The details of experimental settings are provided in Appendix.~\ref{app:sec:detail_observation}.

% 1) Negative transfer: performance degradation caused by multi-task learning in diffusion models, 
% 2) Task affinity: the similarity between gradient directions of denoising tasks across training iterations, which correlated to the performance of a jointly learned model on tasks.
% We use a lightweight ADM~\cite{choi2022perception, dhariwal2021diffusion} and LDM~\cite{rombach2022high} with FFHQ 256$\times$256 dataset~\cite{karras2019style} for analyze diffusion models trained on both pixel and latent space.
% To analyze diffusion models trained on both pixel space and latent space, we use a lightweight variant of ADM~\cite{dhariwal2021diffusion,choi2022perception} and LDM~\cite{rombach2022high} with FFHQ dataset~\cite{karras2019style}.

%\hist{변수만 쓰지 말고, 변수 의미를 되도록 되새김질 ㄱㄱ (e.g., according to timestep $t$)}

%\hist{task affinity 라는 개념이 낯선 편인데, 인용 붙일만한거 없을까여?}
%with task affinity scores~\cite{fifty2021efficiently, azorin2023s}.

% 주의 해야할점 Task affinity scores는 정확하게 Task relationship을 의미하는건 아니에요
% We plot the gradient direction-based task affinity score for each pair of denoising tasks, with the timestep and log-SNR serving as the axes in Fig.~\ref{fig:task_affinity}.
% We plot the gradient direction-based task affinity between denoising task pairs in Fig.~\ref{fig:task_affinity}. 
% In both ADN and LDM, the gradient direction-based task affinity score tends to decrease as the timestep and SNR difference increase, indicating that the directions of gradients from denoising tasks with a large timestep and SNR difference become less similar during the training procedure.
% Also, considering the positive correlation between this score and the performance of the jointly learned model, learning denoising tasks with a large timestep and SNR difference may lead to adverse effects.


% This suggests that diffusion training may benefit from clustering the tasks by the proximity of noise levels, then treating them separately.



% In both ADN and LDM, as the timestep and SNR difference decrease, the affinity score increase, indicating that gradients from denoising tasks with less difference in timestep and nose levels become more similar during training. 
% Furthermore, considering the positive correlation between this score and the model's performance, learning denoising tasks with a large timestep and noise level difference may have small detrimental effects.




% We observe that the gradient direction-based task affinity score tends to decrease as the timestep difference increases in both ADM and LDM. 
% This indicates that the directions of gradients from denoising tasks with a large timestep difference are less similar through the training procedure, and learning them jointly may lead to adverse effects.
% \hist{less similar 에서 adverse effect 로 이어지는게 좀 어색한 것 같아요. making learning them jointly a difficult problem 이라거나... }

% 그 옛날에는 2015 년도 이전 (딥러닝 이전 놈들) MTL을 하는 이유 자체가 그냥 Positive Transfer때문이었대요.
% 긍데, 이제 Negative transfer가 2016년 딥러닝부터는 주로 다뤄짐.
% 혹시 이건 어떠신가여. -> Positive Transfer라는거 일단 안적고, 
% Figure1에서 왼쪽편에 [0, 200]에서는 Positive transfer가 일어나는데,
% 이거 말고 다른 TASK에 대한 Negative transfer를 줄이는게 목표면 되는거 아닐까여? 라는식으로.

% 어캐생각하심? 
% 어떻게 보면 MTL해서 성능 올라갈 수 있기도 하잖아여?
% 긍데 디퓨전짱에서는 Negative transfer짱이 관측된다.?
% ㅠㅠ
% 진영님 Positive transfer도 적어야할까요? 

% 음
% mtl에선 어떻게 전개더ㅣ나여
% 도움이더ㅣ는게 잘알려졋지만 negative가잇다?
% 그럼 만약 쓴대도 맨앞줄에 한줄정도만 해서
% aux테스크 가 tgt 테스크에 도움줄순 잇럿다. 근데 16년부턴 아님 으로 바로 

% fig 1을 해본 이유는 어서 가져오며뉴좋을가여

% ㅇㅎㅇㅎ 그냥 그런데 Negative transfer가 어떤 Task에 있는지 알아본다 정도만 해도 상관없는데, 
% Positive transfer (MTL로 배우면 좋은놈)도 있고 Negative transfer (MTL로 배우면 안좋은놈)도 있음. 긍데 MTL을 잘해서 Negative transfer를 줄이면 성능 올라가는거 아니야? 라고도 할 수 있으니까, 그러게요 그냥 Positive transfer 언급 크게 안하고 넘어가도 될듯하네여...?? 오케이....!
% 오카이! 

% 그렇게해도 nt에 집중하는건 변함없네여!!
% 그림캡션에 적거나 메인에 아주짧게 도음되는경우도잇지만 그 정도가 매우작고 nt가 더 많다 고고고고

% Parameter sharing in multi-task learning can lead to negative transfer, causing performance degradation in some tasks compared to learning them individually~\cite{javaloy2022rotograd, jiang2023forkmerge, ruder2017overview, wang2021gradient}.


% \hyojun{Negative transfer는 competition 때문에 MTL algorithm의 performance가 떨어지는것임.}

% \hyojun{심하면 종종 single task learner의 성능이 MTL의 성능보다 높다는 것임. 그럼 }

% \hyojun{MTL의 benefit도 있는 것임. -> positive한 부분도 주목해봐야함 -> 이걸로 논리를 펴면 안되나?}

% Note that $\Theta(\mathcal{D}^{[0, T]})$ is \textit{multi-task learner} for all denoising tasks and $\Theta(\mathcal{D}^{[t_1, t_2]})$ is \textit{specific-task learner}.
% \jiny{여기에 (footnote) 원래의 NT는 disjoint한 aux와 tgt들을 한번에 학습했을 때 tgt 성능 - tgt만으로 학습한 tgt성능이지만, tgt = [0,T] 이고 aux = [t1,t2]라고 한다면 3번처럼 정의된다라고 명시적인 비유를 일대일로 해주면 어떨까요?}

% \hyojun{Negative transfer gap이라는 용어가 지금 약간 양수일수록 NT가 커지는 것처럼 느껴지는데, 결과는 반대여서 개킹받음 .} \doni{밑에 P가 FID같은거여서 이때는 NTG가 negative일수록 negative transfer가 잘 일어났다라고 설명이 되어있긴 한데, 용어 자체가 주는 혼란이 있으니 말로 설명을 해주더라고 Figure 1 caption에도 다시 한번 언급해주어야 할 듯합니닷. }: 
% Formally, we define the negative transfer gap with a performance measure $P$ as:
% \hist{서로 다른 모델 2개의 성능을 비교한다는걸 처음 보는 사람이 따라가기 어려울 듯 하여... With an introduction of an expert model trained on specific timestep $\mathcal{D}^{[t_1, t_2]}$, we define the gap between the two models as the amount of negative transfer as follows:}

% \hist{$P$ is a performance measurement such as FID...}
% $\Theta(\mathcal{D}^{[t_1, t_2]})$ and $\Theta(\mathcal{D}^{[0, T]})$ respectively denote the model trained on $\mathcal{D}^{[t_1, t_2]}$ and $\mathcal{D}^{[0, T]}$, and

%\hist{이것도 이렇게 하는 이유가 좀 써있어야 할 것 같은데... As the expert model is trained only on the specific timesteps, we leverage the whole model (명칭 맞나) for the other timesteps.}
% Intuitively, the negative transfer gap measures the performance difference between using a model specifically trained on the timestep interval $[t_1, t_2]$ and using a model trained on the entire denoising tasks, within the sampling process.
% \hist{이거 위에 적어놓은 위치에서 잘 버무려야 할 듯. 미괄식 설명이라 여기까지 오기가 어려웠어요.}
% \jiny{FID는 낮을수록 좋으니까, (negative 면 오히려 좋아) 이지 않나요?}
% \hyojun{ Fid(single) - FId (Multi) 여서 Negative면 single task가 좋아서 negative transfer가 발생했다고 봐도 될거같아여}
% \jiny{지금 멀티 - 싱글로 쓰여잇는거 아녜여?제가 먼갈 잘못보고 있으면 알려주세요 죄송 ㅜㅜ}
% With FID score~\cite{heusel2017gans}, if $NTG$ is negative, multi-task learning on $\mathcal{D}^{[0, T]}$ degrades the performance of $\mathcal{D}^{[t_1, t_2]}$ compared that $\mathcal{D}^{[t_1, t_2]}$ is learned individually, indicating that the negative transfer occurs.
% In contrast, positive $NTG$ represents that positive transfer occurs.
% Positive transfer implies that learning entire tasks $\mathcal{D}^{[0, T]}$ is helpful for $\mathcal{D}^{[t_1, t_2]}$ than learning it individually.


% With FID score~\cite{heusel2017gans}, if $NTG$ is negative, the model specifically trained on its timestep interval $\Theta(\mathcal{D}^{[t_1, t_2]})$ outperforms the model trained on entire denoising tasks $\Theta(\mathcal{D}^{[0, T]})$, indicating that the negative transfer occurs.

% We note that our negative transfer measurement differs from previous works~\cite{wang2019characterizing, jiang2023forkmerge} since we cannot evaluate the performance of the model trained on a subset of denoising tasks with sample quality metrics such as FID. 
% Comparison with the negative transfer of previous works is in Appendix~\ref{app:sec:comparison_negative_transfer}.

% \hyojun{여기에 additional 하게는 MTL에서 쓰던 formulation이 살짝 다르다를 언급해도될듯? 이렇게 적을때 생기는 문제는 우리가 정의한 문제를 발견하고 해결하는게 중요한거라는 까임을 당할 수 있음.}
% \hist{negative transfer gain is negative 라는 표현이 뭔가 이상한 것 같아요...}
%\hist{negative transfer gain, negative transfer gap 이 같이 쓰이네요}

% \jiny{그림1에서부터 five parts로 나눌거라면 그림2도 이전에 Line plot으로 그린걸 추가하고 heatmap은 appendix로 뺴보는건 어떨까요?}
% \hyojun{colormap 바까볼게여! }

% This motivates us to leverage well-designed MTL methods since they have addressed the negative transfer.
% \hyojun{ddd}
% \hist{since they have addressed the negative transfer 는 지워도 될 듯?, 앞의 문장에 이어서, which motivates us to leverage well-designed MTL methods. 정도로 이어주면...}



% As shown in the results, both positive transfer and negative transfer occur in diffusion training.


% Alternatively, we use the change in sample quality when using $\Theta(\mathcal{D}^{[t_{1}, t_{2}]})$ on $[t_{1}, t_{2}]$ during sampling of $\Theta(\mathcal{D}^{[0, T]})$, compared to using it throughout the entire sampling process.

% Negative transfer~\cite{ruder2017overview, wang2021gradient, javaloy2022rotograd, jiang2023forkmerge, javaloy2022rotograd} refers to the phenomenon where learning multiple tasks simultaneously can lead to a decrease in performance compared to learning each task individually.
% Using the definitions of~\cite{wang2019characterizing, jiang2023forkmerge}, negative transfer of target denoising tasks in the specific timestep interval $\mathcal{ㄴㄴㄴT}^{[t_{1}, t_{2}]}$ can be measured with performance measure $P$ on $\mathcal{D}^{[t_{1}, t_{2}]}$ as:
% \begin{equation}
%      \label{eq:negative_transfer}
%     NT(\mathcal{D}^{[t_{1}, t_{2}]}) = P(\Theta(\mathcal{D}^{[t_{1}, t_{2}]})) - P(\Theta(\mathcal{D}^{[0, T]})), \quad 0 \leq t_1 \leq t_2 \leq T,
% \end{equation}
% where $\Theta(\mathcal{D}^{[t_{1}, t_{2}]})$ and $\Theta(\mathcal{D}^{[0, T]})$ denote the model trained on $\mathcal{D}^{[t_{1}, t_{2}]}$ and $\mathcal{D}^{[0, T]}$, respectively.
% %\hyojun{여기에 의미 추가 해줘도 될것 같음. ex) 같이 배웠을때의 성능과 하나만 배웠을때의 성능 차이.}
% However, using sample quality metrics such as FID~\cite{} for $P$ in Eq.~\ref{eq:negative_transfer} is challenging because the sample generation of diffusion models requires a learned model covering $\mathcal{D}^{[0, T]}$, and measuring the impact of $\mathcal{D}^{[t_{1}, t_{2}]}$ on sample quality is difficult.
% Alternatively, we use the change in sample quality when using $\Theta(\mathcal{D}^{[t_{1}, t_{2}]})$ on $[t_{1}, t_{2}]$ during sampling of $\Theta(\mathcal{D}^{[0, T]})$, compared to using it throughout the entire sampling process.

% --------------------------------------------------------------------------------

% \paragraph{Negative Transfer Analysis}
% Negative transfer~\cite{ruder2017overview, wang2021gradient, javaloy2022rotograd, jiang2023forkmerge, javaloy2022rotograd} refers to the phenomenon where learning multiple tasks simultaneously can lead to a decrease in performance compared to learning each task individually.
% For the target task $\mathcal{D}_{tgt}$ and auxiliary task $\mathcal{D}_{aux}$, it can be measured with performance measure $P$ on $\mathcal{D}_{tgt}$ as~\cite{wang2019characterizing, jiang2023forkmerge}:
% \begin{equation}
%     \label{eq:negative_transfer_mtl}
%     NT(\mathcal{D}_{aux}, \mathcal{D}_{tgt}) = P(\Theta(\mathcal{D}_{tgt})) - P(\Theta(\mathcal{D}_{tgt}, \mathcal{D}_{aux})),
% \end{equation}
% where $\Theta(\mathcal{D}_{tgt})$ and $\Theta(\mathcal{D}_{tgt}, \mathcal{D}_{aux})$ represent models trained on only $\mathcal{D}_{tgt}$ and on both $\mathcal{D}_{tgt}$ and $\mathcal{D}_{aux}$, respectively.
% For inspecting the negative transfer of denoising tasks $\mathcal{D}^{[t_1, t_2]}$ on timestep range $[t_1, t_2]$ with Eq.~\ref{eq:negative_transfer_mtl}, $\mathcal{D}_{tgt}$ and $\mathcal{D}_{aux}$ might be set as $\mathcal{D}^{[t_1, t_2]}$ and $\mathcal{D}^{[0, T]} \setminus \mathcal{D}^{[t_1, t_2]}$.
% However, sample quality metrics such as FID~\cite{} are not directly compatible with $P$, because sample generation of diffusion models requires the learned model on entire denoising tasks $\mathcal{D}^{[0, T]}$ and measuring the impact of the target task $\mathcal{D}^{[t_{1}, t_{2}]}$ on sample quality is difficult.

% Alternatively, we use the change in sample quality when using $\Theta(\mathcal{D}^{[t_{1}, t_{2}]})$ on $[t_{1}, t_{2}]$ during sampling of $\Theta(\mathcal{D}^{[0, T]})$, compared to using it throughout the entire sampling process.


% --------------------------------------------------------------------------------


% Using the definitions of~\cite{wang2019characterizing, jiang2023forkmerge}, negative transfer of target denoising tasks in the specific timestep interval $\mathcal{D}^{[t_{1}, t_{2}]}$ can be measured with performance measure $P$ on $\mathcal{D}^{[t_{1}, t_{2}]}$ as:
% \begin{equation}
%      \label{eq:negative_transfer}
%     NT(\mathcal{D}^{[t_{1}, t_{2}]}) = P(\Theta(\mathcal{D}^{[t_{1}, t_{2}]})) - P(\Theta(\mathcal{D}^{[0, T]})), \quad 0 \leq t_1 \leq t_2 \leq T,
% \end{equation}
% where $\Theta(\mathcal{D}^{[t_{1}, t_{2}]})$ and $\Theta(\mathcal{D}^{[0, T]})$ denote the model trained on $\mathcal{D}^{[t_{1}, t_{2}]}$ and $\mathcal{D}^{[0, T]}$, respectively.
% %\hyojun{여기에 의미 추가 해줘도 될것 같음. ex) 같이 배웠을때의 성능과 하나만 배웠을때의 성능 차이.}
% However, using sample quality metrics such as FID~\cite{} for $P$ in Eq.~\ref{eq:negative_transfer} is challenging because the sample generation of diffusion models requires a learned model covering $\mathcal{D}^{[0, T]}$, and measuring the impact of $\mathcal{D}^{[t_{1}, t_{2}]}$ on sample quality is difficult.
% Alternatively, we use the change in sample quality when using $\Theta(\mathcal{D}^{[t_{1}, t_{2}]})$ on $[t_{1}, t_{2}]$ during sampling of $\Theta(\mathcal{D}^{[0, T]})$, compared to using it throughout the entire sampling process.


% 따라서 우리는 sampling 과정중 $[t_1, t_2]$ timestep 만 그 task를 배운 individual learner $\Theta(\mathcal{D}^{[t_{1}, t_{2}]})$ 로 대체한 샘플과 일반 sampling에서 생성된 샘플에 대한 quality metric의 차이로 negative transfer를 측정하였습니다.
% 낮은게 좋은 FID와 함께,


% Negative transfer for target task $\mathcal{D}_{tgt}$ with auxiliary task $\mathcal{D}_{aux}$ and performance measure $P$ can be defined as $NT(\mathcal{D}_{tgt}, \mathcal{D}_{aux}) = P(\Theta(\mathcal{D}_{tgt})) - P(\Theta(\mathcal{D}_{tgt}, \mathcal{D}_{aux}))$ in~\cite{wang2019characterizing, jiang2023forkmerge},
% \begin{equation}
%     \label{eq:negative_transfer}
    %NT(\mathcal{D}_{tgt}, \mathcal{D}_{aux}) = P(\Theta(\mathcal{D}_{tgt})) - P(\Theta(\mathcal{D}_{tgt}, \mathcal{D}_{aux})),
% \end{equation}
% where $\Theta(\mathcal{D}_{tgt}, \mathcal{D}_{aux})$ and $\Theta(\mathcal{D}_{tgt})$ denote the model trained on both $\mathcal{D}_{tgt}$ and $\mathcal{D}_{aux}$, and only on $\mathcal{D}_{tgt}$, respectively. 
% For inspecting the negative transfer of denoising tasks in the specific timestep interval $\mathcal{D}^{[t_{min}, t_{max}]}$, $\mathcal{D}_{tgt}$ and $\mathcal{D}_{aux}$ can be respectively set as $\mathcal{D}^{[t_{min}, t_{max}]}$ and $\mathcal{D}^{[t_{min}, t_{max}]}$


% For measuring the negative transfer of denoising tasks in a specific timestep range $[t_{min}, t_{max}]$, $\mathcal{D}_{tgt}$ and $\mathcal{D}_{aux}$ can be set as .
% However, 



==> figure_tex/main_qualitative.tex <==
\captionsetup[sub]{font=scriptsize}
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.098\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figure/qual_result/idx4/input4.png}

         \subcaption{Baseline}
     \end{subfigure}
         \begin{subfigure}[t]{0.098\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figure/qual_result/idx4/warp4.png}

         \subcaption{UW (Timestep)}
     \end{subfigure}
        \begin{subfigure}[t]{0.098\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figure/qual_result/idx4/synsin4.png}


         \subcaption{SynSin~\cite{wiles2020synsin}}
     \end{subfigure}
     \begin{subfigure}[t]{0.098\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Figure/qual_result/idx4/pixelsynth4.png}


     \subcaption{PixelSynth}
    \end{subfigure}
     \begin{subfigure}[t]{0.098\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Figure/qual_result/idx4/geofree4.png}


     \caption{GeoFree~\cite{rombach2021geometry}}
    \end{subfigure}
         \begin{subfigure}[t]{0.098\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Figure/qual_result/idx4/ours4.png}
     \subcaption{Ours}
    \end{subfigure}
    \caption{Qualitative results}
    \label{fig:qual}
\end{figure}

==> figure_tex/overview_algorithm.tex <==
% \begin{figure}
%     \includegraphics[width=\textwidth]{figure_files/interval_clustering.png}
%     \caption{Interval Optimal Clustering \hist{:blobclosefearful:}}
%     \label{fig:interval_clustering}
% \end{figure}






==> macros.tex <==
\newcommand{\todoc}[2]{{\textcolor{#1}{\textbf{#2}}}}
\newcommand{\todoblue}[1]{\todoc{blue}{\textbf{#1}}}
\newcommand{\todored}[1]{\todoc{red}{#1}}
\newcommand{\todobrown}[1]{\todoc{brown}{#1}}
\newcommand{\hyun}[1]{\todoc{purple}{\textbf{hyunseung:} #1}}
\newcommand{\hist}[1]{\todored{\textbf{seungtaek:} #1}}
\newcommand{\hyojun}[1]{\todoblue{\textbf{hyojun:} #1}}
\newcommand{\jiny}[1]{\todobrown{\textbf{jinyoung:} #1}}
\newcommand{\doni}[1]{\todoc{orange}{\textbf{Doni:} #1}}
\newcommand{\yunsung}[1]{\todoc{purple}{\textbf{yunsung:} #1}}

\definecolor{hehe}{rgb}{0, 0.7, 0}
\newcommand{\shinhyeok}[1]{\todoc{hehe}{\textbf{shinhyeok:} #1}}





==> rebuttal/complexity.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}






==> rebuttal/conflict_baseline.tex <==
\begin{figure}[h!]
     \centering
     \includegraphics[width=0.3\textwidth]{rebuttal/figure_file/baseline_conflict.pdf}
     \caption{Average conflict in Baseline}
    \label{fig:behavior_mtl}
\end{figure}

